HOIGaze: Gaze Estimation During Hand-Object Interactions in Extended Reality Exploiting Eye-Hand-Head Coordination

We present HOIGaze - a novel learning-based approach for gaze estimation during hand-object interactions (HOI) in extended reality (XR). HOIGaze addresses the challenging HOI setting by building on one key insight: The eye, hand, and head movements are closely coordinated during HOIs and this coordination can be exploited to identify samples that are most useful for gaze estimator training - as such, effectively denoising the training data. This denoising approach is in stark contrast to previous gaze estimation methods that treated all training samples as equal. Specifically, we propose: 1) a novel hierarchical framework that first recognises the hand currently visually attended to and then estimates gaze direction based on the attended hand; 2) a new gaze estimator that uses cross-modal Transformers to fuse head and hand-object features extracted using a convolutional neural network and a spatio-temporal graph convolutional network; and 3) a novel eye-head coordination loss that upgrades training samples belonging to the coordinated eye-head movements. We evaluate HOIGaze on the HOT3D and Aria digital twin (ADT) datasets and show that it significantly outperforms state-of-the-art methods, achieving an average improvement of 15.6% on HOT3D and 6.0% on ADT in mean angular error. To demonstrate the potential of our method, we further report significant performance improvements for the sample downstream task of eye-based activity recognition on ADT. Taken together, our results underline the significant information content available in eye-hand-head coordination and, as such, open up an exciting new direction for learning-based gaze estimation.

==> sections/figures_only.tex <==
% figures, [htbp] is used to set the format of our figures.
\begin{figure*}[t]
    \centering
    \subfloat[HOT3D (Cross-User)]{\includegraphics[width=0.33\linewidth]{assets/hot3d_user.pdf}} 
    \subfloat[HOT3D (Cross-Scene)]{\includegraphics[width=0.33\linewidth]{assets/hot3d_scene.pdf}}
    \subfloat[ADT]{\includegraphics[width=0.33\linewidth]{assets/adt.pdf}}
    \caption{The cumulative distribution functions of different methods' estimation errors on HOT3D (Cross-User), HOT3D (Cross-Scene), and ADT. The higher the CDF curve, the better the performance. Our method achieves better performance than other methods in terms of estimation error distributions.} \label{fig:error_distribution}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{assets/results.png}
    \caption{Visualisation of the gaze estimation results from our method and the state-of-the-art method \textit{Pose2Gaze}~\cite{hu24pose2gaze} on the HOT3D dataset. The green arrow represents the ground truth eye gaze, the red arrow denotes our method, the blue arrow refers to \textit{Pose2Gaze}. Our method exhibits higher estimation accuracy than the state-of-the-art method at different scenarios and different activities.}\label{fig:results}
\end{figure*}
